H\"older estimates for fractional parabolic equations with critical divergence free drifts

This work focuses on drift-diffusion equations with fractional dissipation $(-\Delta)^{\alpha}$ in the regime $\alpha \in (1/2,1)$. Our main result is an a priori H\"older estimate on smooth solutions to the Cauchy problem, starting from initial data with finite energy. We prove that for some $\beta \in (0,1)$, the $C^{\beta}$ norm of the solution depends only on the size of the drift in critical spaces of the form $L^{q}_{t}(BMO^{-\gamma}_{x})$ with $q>2$ and $\gamma \in (0,2\alpha-1]$, along with the $L^{2}_{x}$ norm of the initial datum. The proof uses the Caffarelli/Vasseur variant of De Giorgi's method for non-local equations.

==> Cacciop_IterLem.tex <==
%!TEX root = main.tex

{\color{red} Move this to an appendix?}

\begin{Lem}\label{L.IterationLemma}
Let $\phi: [r_{1},r_{2}] \times [\delta_{1},\delta_{2}] \to \R_{+}$ be a positive, bounded function which is monotone in the two parameter sense.  Let $A_{1} \in \R$, $A_{2} \in \R_{+}$ be constants and $\beta_{1},\beta_{2} \in \R_{+}$ be exponents. 

Assume there exists a $\kappa \in (0,1)$ with the following property.  For all $r_{2}<r<R<r_{2}$ and $\delta_{1}<\delta<\rho<\delta_{2}$ $:$
\begin{equation}
\phi(r,\delta) \leq A_{1}+\frac{A_{2}}{(\delta-\rho)^{\beta_{1}}(R-r)^{\beta_{2}}}+\kappa \phi(R,\rho).
\end{equation}
Then there exists a constant $C(\kappa)$ depending solely on $\kappa$, such that:
\begin{equation}
\phi(r_{1},\delta_{1}) \leq C(\kappa) \left( A_{1}+\frac{A_{2}}{(\delta_{2}-\delta_{1})^{\beta_{1}}(r_{2}-r_{1})^{\beta_{2}}} \right).
\end{equation}
\end{Lem}




==> Cacciop_ProdEst.tex <==
%!TEX root = main.tex
For the proof of Proposition~\ref{P.CacciopioliInequality}, we need a few estimates on the product of $BMO^{-\gamma}$ space.

\begin{Lem}\label{L.BMOProd} \marginnote{Slightly inconsistent to use $\gamma/2$ here rather than $\gamma$}
For all $p \in (1,\infty)$ and $\gamma \in (0,1)$, there exists a positive constant $C_{p,\gamma}$ such that the following is true.  For each $f \in C^{\infty}(\R^{d}) \cap BMO^{-\gamma}(\R^{d})$ and $g \in C_{c}(\R^{d}) \cap W^{1,\infty}(\R^{d})$ supported in $B_{1}$,
\begin{equation}\label{E.BMOProd}
\int_{\R^{d}}fg\dx \leq C_{p,\gamma}\|f\|_{BMO^{-\gamma}(\R^{d})}\bigg [ \big\|(-\Delta)^{\frac{\gamma}{2}}g \big\|_{L^{p}(\R^{d})}+\|g\|_{L^{1}(\R^{d})}\bigg].
\end{equation}
\end{Lem}
Note that the reason for the lipschitz regularity in the propsition above is that we apply it to $\theta_{+}$.  Perhaps we should clarify that the constant also depends on the support of $g$ I think?
\begin{Prop} \label{P.ClassicalBMO} 
For all $p \in (1,\infty)$, there exists a positive constant $C_{p}$ such that for each \linebreak $\psi \in BMO(\R^{d})$,
\begin{align*}
\|\psi-M(\psi,B_{2})\|_{L^{p}(B_{2})}\leq C_{p}\|\psi\|_{BMO(B_{2})}.
\end{align*} 
Moreover, for all $\gamma \in (0,2)$, there exists a positive constant $C_{\gamma}$ such that:
\begin{align*}
\int_{\R^{d}}\frac{|\psi-M(\psi,B_{2})|}{2^{d+\gamma}+|x|^{d+\gamma}}\dx \leq C_{\gamma}\|\psi\|_{BMO(\R^{d})},
\end{align*}
where
$$
M(\psi,B_{2})=\frac{1}{|B_{2}|}\int_{B_2}\psi \dx.
$$
\end{Prop}


\begin{Lem} \label{L.AwayFromSupport}
For each $\gamma \in (0,1)$, there exists a positive constant $C_{\gamma}$ with the following property.  For all $g \in C_{c}(\R^{d}) \cap W^{1,\infty}(\R^{d})$ supported in $B_{1}$ and each $x \in B_{2}^{c}$,
\begin{align*}
\big|(-\Delta)^{\frac{\gamma}{2}}g(x)\big| \leq C_{\gamma}\|g\|_{L^{1}(B_{1})}\big ( 1+|x|^{d+\gamma} \big )^{-1}.
\end{align*}
In particular, $(-\Delta)^{\frac{\gamma}{2}}g \in L^{1}(\R^{d})$ and satisfies:
$$
\int_{\R^{d}}(-\Delta)^{\frac{\gamma}{2}}g(x)\dx = 0.
$$
\end{Lem}
\begin{proof}
Let $x \in B_{2}^{c}$, then since $g$ is compactly supported in $B_{1}$
\begin{equation} \label{eq:fracLapAwayFromSupp}
(-\Delta)^{\frac{\gamma}{2}}g(x)=c_{\gamma}\int_{B_{1}}\frac{g(y)}{|x-y|^{d+\gamma}}\dee y,
\end{equation}
where the integral is absolutely convergent.  Moreover, for $y \in B_{1}$ we have the elementary inequality
\begin{equation} \label{eq:ElemIneq}
|x-y| \geq |x|-|y|=\frac{1}{3}|x|+\bigg(\frac{2}{3}|x|-|y|\bigg) \geq \frac{1}{3}(1+|x|).
\end{equation}
Combining \eqref{eq:fracLapAwayFromSupp} and \eqref{eq:ElemIneq} gives the claim.
\end{proof}


\begin{proof}[Proof of Lemma \ref{L.BMOProd}] \,Begin by writing $f=(-\Delta)^{\frac{\gamma}{2}}\psi$ and applying Lemma \ref{L.FractionalIBP} to find:
$$
\int_{\R^{d}}fg\dx = \int_{\R^{d}}\psi (-\Delta)^{\frac{\gamma}{2}}g\dx.
$$
By Lemma \ref{L.AwayFromSupport}, $(-\Delta)^{ \frac{\gamma}{2} }g$ integrates to zero over $\R^{d}$.  We may exploit this by introducing:
$$
\psi_{0}(x)=\psi(x)-M(\psi,B_{2}).
$$
A free subtraction yields:
\begin{align*}
\int_{\R^{d}}fg\dx = \int_{\R^{d}}\psi_{0} (-\Delta)^{\frac{\gamma}{2}}g\dx 
=\int_{B_{2}}\psi_{0} (-\Delta)^{\frac{\gamma}{2}}g\dx+\int_{B_{2}^{c}}\psi_{0} (-\Delta)^{\frac{\gamma}{2}}g\dx.
\end{align*}
To estimate the inner contribution, apply H\"{o}lder's inequality followed by Proposition \ref{P.ClassicalBMO} to obtain: 
\begin{align*}
\int_{B_{2}}\psi_{0} (-\Delta)^{\frac{\gamma}{2}}g\dx &\leq \|\psi_{0}\|_{L^{\frac{p}{p-1}}(B_{2})}\big \|(-\Delta)^{\frac{\gamma}{2}}g\big \|_{L^{p}(\R^{d})}\\
& \leq C_{p}\|\psi\|_{BMO(\R^{d})}\big \|(-\Delta)^{\frac{\gamma}{2}}g\big \|_{L^{p}(\R^{d})}. 
\end{align*}
To estimate the outer contribution, use Lemma \ref{L.AwayFromSupport} (noting that $g$ is compactly supported in $B_{1}$) followed by Proposition \ref{P.ClassicalBMO} to deduce
\begin{align*}
\int_{B_{2}^{c}}\psi_{0} (-\Delta)^{\frac{\gamma}{2}}g\dx &\leq C_{\gamma}\|g\|_{L^{1}(B_{1})}  \int_{\R^{d}}\frac{|\psi(x)-M(\psi,B_{2})|}{1+|x|^{d+\gamma}}\dx \\
&\leq C_{\gamma} \|g\|_{L^{1}(B_{1})} \int_{\R^{d}}\frac{|\psi(x)-M(\psi,B_{2})|}{ 2^{d+\gamma}+|x|^{d+\gamma}}\dx \\
&\leq C_{\gamma}\|g\|_{L^{1}(B_{1})}\|\psi\|_{BMO(\R^{d})}.
\end{align*}
The proof of the Lemma is completed in view of the observation $\|\psi\|_{BMO(\R^{d})}=\|f\|_{BMO^{-\gamma}(\R^{d})}$.
\end{proof}


==> Cacciop_Proof.tex <==
%!TEX root = main.tex

\begin{proof}[Proof of Proposition~\ref{P.CacciopioliInequality}]
Missing


First, we reduce the Proposition to estimating the drift term.
%\begin{Rem}
%We can compute the exponent $\frac{q}{q-2}$ in terms of $\alpha, \gamma >0$ as follows.  Recall that $\frac{2\alpha}{q}+\gamma = 2\alpha -1$, so that $\frac{2\alpha}{q}=2\alpha -1 - \gamma$.  Solving for $q$ yields $q=\frac{2\alpha}{2\alpha-1-\gamma}$.  Moreover, we may compute $q-2 = \frac{2\alpha-2(2\alpha-1-\gamma)}{2\alpha-1-\gamma}$.  Taking the ratio and cancelling a term gives $\frac{q}{q-2}=\frac{2\alpha}{2(1+\gamma)-2\alpha}=\frac{\alpha}{1+\gamma-\alpha}$.
%\end{Rem}
\begin{Lem}
%For each $\theta \in \mathcal{S}(D,\alpha)$ driven by $u: \R_{+} \times \R^{d} \to \R$,
Under the hypotheses of Proposition \ref{P.CacciopioliInequality}, the following inequality holds true.
\begin{equation}\label{E.ReductionToDrift}
\begin{split}
\|\eta \theta_{+}(t)\|_{L^{2}(\R^{d})}^{2}&+2\int_{s}^{t}\|\nabla \big (\sigma \theta_{+}^{*}(r) \big )\|^{2}_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})}\dee r
\leq \|\eta \theta_{+}(s)\|_{L^{2}(\R^{d})}^{2} \\
&+ 2\int_{s}^{t}\|\nabla \sigma \theta_{+}^{*}(r)\|^{2}_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})}\dee r+\int_{s}^{t}\|u(r)\cdot \nabla(\eta^{2})\theta_{+}^{2}(r)\|_{L^{1}(\R^{d})}\dee r.
\end{split}
\end{equation}
\end{Lem}

\begin{proof}
Multiplying the equation for $\theta \in \mathcal{S}(D,\alpha)$ by $\eta^{2}\theta_{+}$ and integrating over $[s,t] \times \R^{d}$ yields:
\begin{equation} \label{E.LocalizeIBP}
\begin{split}
&\frac{1}{2}\int_{\R^{d}}\theta_{+}^{2}(t,x)\eta^{2}(x)\dx + \int_{s}^{t}\int_{\R^{d}} (-\Delta)^{\alpha}\theta \eta^{2}\theta_{+} \dx\dee r\\
&= \frac{1}{2}\int_{\R^{d}}\theta_{+}^{2}(s,x)\eta^{2}(x)\dx - \frac{1}{2}\int_{s}^{t}\int_{\R^{d}} u \cdot \nabla(\theta_{+}^{2}) \eta^{2} \dx\dee r.
\end{split}
\end{equation}
Since $\Div u = 0$, we may write:
\begin{align}\label{E.DivFree}
&- \frac{1}{2}\int_{s}^{t}\int_{\R^{d}} u \cdot \nabla(\theta_{+}^{2}) \eta^{2} \dx\dee r
=\frac{1}{2}\int_{s}^{t}\int_{\R^{d}} u \cdot \nabla(\eta^{2})\theta_{+}^{2}\dx\dee r.
\end{align}
Next we will verify that for all times in $[s,t]$,
\begin{equation}\label{E.LiftToUHP}
\int_{\R^{d}} (-\Delta)^{\alpha}\theta \eta^{2} \theta_{+} \dee x = \int_{\R^{d}}\int_{0}^{\infty}z^{1-2\alpha}\bigg ( |\nabla(\sigma\theta_{+}^{*})|^{2}-|\nabla \sigma|^{2}|\theta_{+}^{*}|^{2} \bigg)\dx \dee z.
\end{equation}
Applying Lemma \ref{L.FundamentalIdentity} with $f = \theta$, $g = \eta^{2} \theta_{+}$ and the extension $\overline{g}=\sigma^{2}\theta_{+}^{*}$,
\begin{align*}
\int_{\R^{d}} (-\Delta)^{\alpha}\theta \eta^{2} \theta_{+} \dx &= \int_{0}^{\infty}\int_{\R^{d}} z^{1-2\alpha}\nabla(\sigma^{2}\theta_{+}^{*}) \cdot \nabla \theta^{*}\dx\dee z \\
& = \int_{0}^{\infty}\int_{\R^{d}} z^{1-2\alpha}\nabla(\sigma^{2}\theta_{+}^{*}) \cdot \nabla \theta_{+}^{*}\dx\dee z.
\end{align*}
The identity \eqref{E.LiftToUHP} now follows from the relation 
$$
\nabla(\sigma^{2}\theta_{+}^{*}) \cdot \nabla \theta^{*}_{+} = |\nabla(\sigma \theta^{*}_{+})|^{2}-|\nabla \sigma|^{2}|\theta^{*}_{+}|^{2}.
$$
Substituting the identities \eqref{E.DivFree} and \eqref{E.LiftToUHP} into \eqref{E.LocalizeIBP} and multiplying by a factor of $2$ yields the desired identity \eqref{E.ReductionToDrift}.
\end{proof}

It is worth pointing out that the estimate below, which is a sort of localized version of the BMO product lemma, is the source of the bad term which we ultimately must iterate away. Note also that it is important for us that $\gamma<\alpha$ here since we are effectively using that $\epsilon$ trick from an earlier draft.

\begin{Lem}\label{L.DriftEstimate}
For each $\gamma \in (0,\alpha)$ there exists a positive constant $C_{\gamma,\alpha}$ with the following property.  For all $u \in C^{\infty}(\R^{d}) \cap BMO^{-\gamma}(\R^{d})$, $\theta \in C^{\infty}(\R^{d})$, and $\sigma \in C^{\infty}_{c}\big(B_1\times [0,\infty) \big)$, the inequality below holds true:
\begin{align*}
\left | \int_{\R^{d}}u \cdot \eta \nabla \eta \theta_{+}^{2}\dee x \right |
&\leq C_{\gamma,\alpha}\nu^{-1}\|u\|_{BMO^{-\gamma}(\R^{d})}^{2}\|(\eta + |\nabla \eta|)\theta_{+}\|^{2}_{L^{2}(\R^{d})}\\
&+\|\nabla(\sigma \theta^{*}_{+})\|_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})}+\nu \|\nabla(\nabla_{x} \sigma \theta_{+}^{*})\|^{2}_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})},
\end{align*}
where $\nu \in (0,1)$ is arbitrary and $\eta(x)=\sigma(x,0)$.
\end{Lem}

\begin{proof}
Let $f=u$ and $g=\eta \nabla \eta\theta_{+}^{2}$.  Since $\theta \in C^{\infty}(\R^{d})$, it follows that $g \in C_{c}(\R^{d}) \cap W^{1,\infty}(\R^{d})$.  Hence, we may apply Lemma \ref{L.BMOProd} with an exponent $p(\alpha,\gamma) \in (1,2)$ to be chosen below.  This yields:
\begin{equation}
\int_{\R^{d}}u \cdot \eta \nabla \eta \theta_{+}^{2}\dx \leq C_{\gamma,\alpha}\|u\|_{BMO^{-\gamma}(\R^{d})}\bigg [ \|\eta \nabla \eta \theta_{+}^{2}\|_{L^{1}(\R^{d})}+\big \|(-\Delta)^{\frac{\gamma}{2}}(\eta \nabla \eta \theta_{+}^{2})\big \|_{L^{p}(\R^{d})} \bigg].
\end{equation}
To estimate the first term, use Young's inequality to find:
\begin{equation}
\|u\|_{BMO^{-\gamma}(\R^{d})} \|\eta \nabla \eta \theta_{+}^{2}\|_{L^{1}(\R^{d})}
\leq \frac{1}{2}\big[1+\|u\|_{BMO^{-\gamma}(\R^{d})}^{2} \big ]\|(\eta + |\nabla \eta|)\theta_{+}\|_{L^{2}(\R^{d})}^{2}.
\end{equation}
The next step is to apply Kato-Ponce's inequality (Theorem \ref{T.KatoPonce}) to $\eta \theta_{+}$ and $\nabla \eta \theta_{+}$ to obtain:
\begin{align*}
&\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+} \nabla \eta \theta_{+})\big\|_{L^{p}(\R^{d})}\\
&\leq C_{\gamma}\bigg [ \big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{\frac{2p}{2-p}}(\R^{d})}\|\nabla \eta \theta_{+}\|_{L^{2}(\R^{d})}+\|\eta \theta_{+}\|_{L^{2}(\R^{d})}\big\|(-\Delta)^{\frac{\gamma}{2}}(\nabla \eta \theta_{+})\big \|_{L^{\frac{2p}{2-p}}(\R^{d})} \bigg].
\end{align*}
\marginnote{Perhaps treat the case of dimension one separately here since otherwise i think we need dimension larger than 2}Since $\alpha>\gamma$, we may choose the exponent $p=d/(\alpha-\gamma)$ 

{\color{blue}(actually it should be $p=\frac{d}{d-(\alpha-\gamma)}<2$)
The equation it solves it should be
$$
\frac{2p}{p-2}=\frac{2d}{d-2(\alpha-\gamma)}.
$$


}




which is larger than $2$ since $\gamma>0$, $\alpha<1$ and $d \geq 2$. This allows us to use the Hardy-Littlewood-Sobolev inequality to deduce 
\begin{align*}
&\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+} \nabla \eta \theta_{+})\big\|_{L^{p}(\R^{d})}\\
&\leq C_{\gamma}\bigg [ \big\|(-\Delta)^{\frac{\alpha}{2}}(\eta \theta_{+})\big \|_{L^{2}(\R^{d})}\|\nabla \eta \theta_{+}\|_{L^{2}(\R^{d})}+\|\eta \theta_{+}\|_{L^{2}(\R^{d})}\big \|(-\Delta)^{\frac{\alpha}{2}}(\nabla \eta \theta_{+})\big \|_{L^{2}(\R^{d})} \bigg].
\end{align*}
Combining these observations and using Young's inequality with a parameter $\nu>0$, we find:
\begin{align*}
\int_{\R^{d}}u \cdot \eta \nabla \eta \theta_{+}^{2}\dx &\leq C_{\gamma}\nu^{-1}\bigg[1+\|u\|_{BMO^{-\gamma}(\R^{d})}^{2} \bigg ]\|(\eta + |\nabla \eta|)\theta_{+}\|^{2}_{L^{2}(\R^{d})}\\
&+\big \|(-\Delta)^{\frac{\alpha}{2}}(\eta \theta_{+})\big \|^{2}_{L^{2}(\R^{d})}+\nu \big \|(-\Delta)^{\frac{\alpha}{2}}(\nabla \eta \theta_{+})\big \|^{2}_{L^{2}(\R^{d})}.
\end{align*}
The proof may be completed by using the variational characterization of the $\dot{H}^{\alpha}$ norm, Proposition \ref{prop:variational}.  Namely, choose $\sigma \theta_{+}^{*}$ to extend $\eta \theta_{+}$ and $\nabla_{x} \sigma \theta_{+}^{*}$ to extend $\nabla \eta \theta_{+}$.
\end{proof}
{\color{blue}
Let's try to fix this proof. If I follow the proof correctly, as it is, it would force us to take $p=d/(\alpha-\gamma)$, which contradicts the hypothesis of the Kato-Ponce. For Kato-Ponce to work, we need $p<2$.

The question is if we have the bound
$$
\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{\frac{2p}{2-p}}(\R^{d})}
\le
C_{\gamma}\left[
\|(-\Delta)^{\frac{\alpha}{2}}(\eta \theta_{+})\big \|_{L^{2}(\R^{d})}
+
\|\eta \theta_{+}\|_{L^{2}(\R^{d})}
\right]
$$
For now, let's call $\frac{2p}{2-p}=q$, which is always above $2$ and can be chosen to be as close as we need.

To prove the desired inequality, the first step is to take care of the far field, by applying Lemma~\ref{L.AwayFromSupport}:
$$
\begin{aligned}
\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{q}(B_2^c)}&
\le  ||C_\gamma \|\eta \theta_{+}\|_{L^{1}(\R^{d})}(1+|x|^{d+\gamma})^{-1}||_{L^q(B_2^c)}\\
&\le C_\gamma \|\eta \theta_{+}\|_{L^{1}(\R^{d})}\le C_\gamma \|\eta \theta_{+}\|_{L^{2}(\R^{d})},
\end{aligned}
$$
where in the last inequality we have used that the support of $\eta \theta_{+}$ is contained in $B_1$.

For the other part we just apply H\"{o}lder to raise the homogeneity of the norm
$$
\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{q}(B_2)}\le C\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{r}(B_2)}\le C\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{r}(\R^d)} ,
$$
where $r=\frac{2d}{d-2(\alpha-\gamma)}>q>2$. Finally, $r$ has been chosen, to be able to apply the Hardy-Littlewood-Sobolev inequality, therefore
$$
\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{q}(B_2)}
\le
C\big\|(-\Delta)^{\frac{\gamma}{2}}(\eta \theta_{+})\big\|_{L^{r}(\R^d)}
\le
\|(-\Delta)^{\frac{\alpha}{2}}(\eta \theta_{+})\big \|_{L^{2}(\R^{d})}.
$$
}




Now we are in a position to complete the proof of Propsition \ref{P.CacciopioliInequality}.
\begin{proof}[Proof of Proposition \ref{P.CacciopioliInequality}]
Fix a $\nu>0$ and apply Lemma \ref{L.DriftEstimate} for each time in $r \in (s,t)$ to find
\begin{align*}
\int_{s}^{t}\int_{\R^{d}}u \cdot \eta \nabla \eta \theta_{+}^{2}\dx \dee r &\leq C_{\gamma}\nu^{-1}\int_{s}^{t}\|u(r)\|_{BMO^{-\gamma}(\R^{d})}^{2}\|(\eta + |\nabla \eta|)\theta_{+}(r)\|^{2}_{L^{2}(\R^{d})}\dee r\\
&+\int_{s}^{t}\|\nabla(\sigma \theta^{*}_{+})\|^{2}_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})}\dee r+\nu \int_{s}^{t}\|\nabla(\nabla \sigma \theta_{+}^{*})\|^{2}_{L^{2}_{\omega_{\alpha}}(\R^{d} \times \R_{+})}\dee r.
\end{align*}
Recall that $u \in L^{q}_{t}(BMO^{-\gamma})$, where the exponent $q$ and $\gamma$ satisfy $\frac{2\alpha}{q}+\gamma=2\alpha-1$.  Since $\gamma>0$, it follows that $q$ is at least as large as $2\alpha/(2\alpha-1)$.  Hence, applying Holder's inequality with the exponent $\alpha/(2\alpha-1)$ yields:
\begin{align*}
&\int_{s}^{t}\bigg[1+\|u(r)\|_{BMO^{-\gamma}(\R^{d})}^{2}\bigg]\|(\eta + |\nabla \eta|)\theta_{+}(r)\|^{2}_{L^{2}(\R^{d})}\dee r \\ 
&\leq \bigg ( \int_{s}^{t}\bigg[1+\|u(r)\|_{BMO^{-\gamma}(\R^{d})}^{2}\bigg]^{\frac{\alpha}{2\alpha-1}}\dee r \bigg )^{2-\frac{1}{\alpha}} \bigg ( \int_{s}^{t}\|(\eta + |\nabla \eta|)\theta_{+}(r)\|^{\frac{2\alpha}{1-\alpha}}_{L^{2}(\R^{d})}\dee r \bigg )^{\frac{1}{\alpha}-1}\\
&\leq C(D,\alpha) \bigg ( \int_{s}^{t}\|(\eta + |\nabla \eta|)\theta_{+}(r)\|^{\frac{2\alpha}{1-\alpha}}_{L^{2}(\R^{d})}\dee r \bigg )^{\frac{1}{\alpha}-1},
\end{align*}
where in the last inequality we used Holder once more since $2\alpha/(2\alpha-1)<q$ and $s,t<2$.  Combining these observations with \eqref{E.ReductionToDrift} completes the proof.
\end{proof}
Intuitively, the way to remember how to get the exponent is that we must consider when $q$ is at its minimum, corresponding to $\gamma=0$ since we can only lower $q$ (and making the problem more super-critical) at the expense of lowering $\gamma$.
\end{proof}

==> ScalingRed.tex <==
%!TEX root = main.tex
Our first theorem can be stated as follows:
\begin{Thm} \label{Thm:HolderContResult}
For all $r>0$, there exist positive constants $\beta, C$ such that for all $\theta \in \mathcal{S}(D,\alpha)$ with $\theta(0) \in L^{2}(\R^{d})$, 
\begin{equation}
|\theta|_{C^{\beta} ( [r,\infty) \times \R^{d} )} \leq C r^{-2\alpha d}|\theta(0)|_{L^{2}(\R^{d})}.
\end{equation}
Moreover, the constants $\beta,\;C$ are universal(depend only on $D$ and $\alpha$).
\end{Thm}
We prove Theorem~\ref{Thm:HolderContResult} by using the standard De Giorgi iterarion, which starts with the $L^{2}_{x}(\R^d) \to L^{\infty}_{x}(\R^d)$ step.  Namely, we have the following consider the following Lemma
\begin{Lem} \label{L.L2toLinfWholeSpace}
There exists a universal constant $C(d,\alpha)$ with the following property. For all $\theta \in \mathcal{S}(D,\alpha)$ with $\theta(0) \in L^{2}(\R^{d})$ and every time $t_{0}>0$, the estimate below holds true:
\begin{equation}
|\theta |_{L^{\infty}([t_{0},\infty] \times \R^{d})} \leq C |\theta(0)|_{L^{2}(\R^{d})}t_{0}^{-2\alpha d}.
\end{equation}
\end{Lem}
\begin{Rem}
The constant $C$ in Lemma \ref{L.L2toLinfWholeSpace} is independent of the size of the critical drift $D$.
\end{Rem}

\begin{proof}
Let us begin by reducing the Lemma to a proof of the following claim:
\begin{Claim}\label{Claim.ScalingRedLinf}
There exists a positive $\epsilon_{0}(\alpha,d)$ with the following property.  If $\theta \in \mathcal{S}(D,\alpha)$ and $|\theta(0)|_{L^{2}(\R^{d})}^{2}\leq \epsilon_{0}$, then
$$
|\theta|_{L^{\infty}([1,\infty] \times \R^{d})} \leq 1.
$$
\end{Claim}
Assuming the claim, let us complete the proof. Let $\theta \in S(D,\alpha)$ and $\theta(0) \in L^{2}(\R^{d})$.  For each time $t_{0}>0$, we truncate and rescale and define $\tilde{\theta} \in \mathcal{S}(D,\alpha)$ via:
\begin{equation}
\tilde{\theta_+}(t,x)=\epsilon_{0}^{\frac{1}{2}}|\theta(0)|_{L^{2}(\R^{d})}^{-1}\theta(t_{0}t,t_{0}^{\frac{1}{2\alpha}}x).
\end{equation}
Applying the claim to $\tilde{\theta}$ and undoing the scaling gives:
\begin{equation}\label{eq:Einfty}
|\theta|_{L^{\infty}([t_{0},\infty] \times \R^{d})} \leq \epsilon_{0}^{-\frac{1}{2}} |\theta(0)|t_{0}^{-2\alpha d}.
\end{equation}
Setting $C=2\epsilon_{0}^{-\frac{1}{2}}$ completes the proof of the Lemma.  Hence, it suffices to prove Claim \eqref{Claim.ScalingRedLinf}.

\end{proof}

\begin{proof}[Proof of Claim~\ref{Claim.ScalingRedLinf}] 
We prove the claim by proving that $\epsilon_{0}>0$ sufficiently small,
\begin{equation} \label{eq:ZeroTrunc}
||(\theta-1)_+||^{2}_{L^{\infty}([1,\infty);L^{2}(\R^{d})}=0
\end{equation}
Applying this observation to both $\theta$ and $-\theta$ completes the proof of the claim.

For each $k \in \N_{0}$,  we define:
\begin{itemize}
\item $T_{k}=1-2^{-k}$ a time cut,
\item $M_{k}=1-2^{-k}$ a level,
\item $\theta_{k}=(\theta - M_{k})_{+}$ the corresponding truncation,
\item $E_{k}=||\theta_{k}||^{2}_{L^{\infty}([T_{k},\infty);L^{2}(\R^{d})}+|\theta_{k}|^{2}_{L^{2}([T_{k},\infty];H^{\alpha}(\R^{d}))}$ the corresponding energy.
\end{itemize}


Our goal is to establish a nonlinear recursive relation between the energy at step $k$ and the energy at step $k-1$.  The first point is to observe that for all times $0 \leq s < t$ by Lemma~\ref{lem:firstenergyinequality}, we know that
\begin{equation} \label{E.EnergyIneq}
\frac{1}{2}|\theta_{k}(t)|_{L^{2}(\R^{d})}^{2} + |\theta_{k}|^{2}_{L^{2}([s,t];\dot{H}^{\alpha}(\R^{d}))} \leq \frac{1}{2}|\theta_{k}(s)|_{L^{2}(\R^{d})}^{2}.
\end{equation}

The next point is to apply \eqref{E.EnergyIneq} in two different ways.  First we work with $k=s=0$ and maximize over $t>0$ to find.
\begin{equation} \label{E.IniitalSmallness}
\begin{split}
E_{0} &\leq |\theta_{+}|_{L^{\infty}([1/2,\infty);L^{2}(\R^{d}))}^{2} + |\theta_{+}|_{L^{2}([1/2,\infty);\dot{H}^{\alpha}(\R^{d}))}^{2} \\
 &\leq 2|\theta_{+}(0)|_{L^{2}(\R^{d})}^{2} \leq 2\epsilon_{0}.
\end{split}
\end{equation}
The second application of \eqref{E.EnergyIneq} is with an arbitrary $k \in \N$.  Fixing an $s \in [T_{k-1},T_{k}]$ then maximizing over $t \in [T_{k},\infty)$ yields 
$$
E_{k}\leq 2|\theta_{k}(s)|_{L^{2}(\R^{d})}^{2}\;\;\;\;\forall s\in[T_{k-1},T_{k}]
$$
Averaging this inequality over $s$ we find:
\begin{equation} \label{E.InitialEnergyBound}
E_{k}
\leq\min_{s\in[T_{k-1},T_{k}]} 2|\theta_{k}(s)|_{L^{2}(\R^{d})}^{2}
\leq \frac{1}{{T_{k}-T_{k-1}}}\int_{T_{k-1}}^{T_{k}} 2|\theta_{k}(t)|_{L^{2}(\R^{d})}^{2}\;dt
\leq 2^{k+1}|\theta_{k}|^{2}_{L^{2}([T_{k-1},\infty) \times \R^{d})}.
\end{equation}

The next step is to interpolate and use a Sobolev embedding to find:
\begin{equation} \label{E.Interpolate}
\begin{split}
&|\theta_{k-1}|_{L^{2+\frac{4\alpha}{d}}\big ([T_{k-1},\infty) \times \R^{d}\big )} 
\leq |\theta_{k-1}|_{L^{\infty} \big ([T_{k-1},\infty);L^{2}(\R^{d})\big)}^{\frac{2\alpha}{d+2\alpha}}
|\theta_{k-1}|_{L^{2} \big ([T_{k-1},\infty);L^{\frac{2d}{d-2\alpha}}(\R^{d})\big)}^{\frac{d}{d+2\alpha}}\\
& \leq E_{k-1}^{\frac{\alpha}{d+2\alpha}}|\theta_{k-1}|_{L^{2} \big ([T_{k-1},\infty);\dot{H}^{\alpha}(\R^{d})\big)}^{\frac{d}{d+2\alpha}}\leq E_{k-1}^{\frac{1}{2}}.
\end{split}
\end{equation}
Observe that if $\theta_{k}(t,x)>0$, then $\theta_{k-1}(t,x) > 2^{-k}$.  Hence, $1_{\{ \theta_{k}>0 \}}\leq 2^{\frac{4\alpha k}{d}}\theta_{k-1}^{\frac{4\alpha}{d}}$.  Combining this observation with inequalities \eqref{E.InitialEnergyBound} and \eqref{E.Interpolate}, we find that:
\begin{equation} \label{E.NonLinearIneq}
\begin{split}
E_{k} &\leq 2^{k+1}|\theta_{k}1_{\{\theta_{k}>0\}}|^{2}_{L^{2}([T_{k-1},\infty] \times \R^{d})}\\
& \leq 2^{(\frac{4\alpha}{d}+1)k+1} |\theta_{k-1}|_{L^{2+\frac{4\alpha}{d}}\big ([T_{k-1},\infty) \times \R^{d}\big )}^{2+\frac{4\alpha}{d}}\\
& \leq 2^{(\frac{4\alpha}{d}+1)k+1} E_{k-1}^{1+\frac{2\alpha}{d}}.
\end{split}
\end{equation}
The Claim now follows from \eqref{E.IniitalSmallness} and \eqref{E.NonLinearIneq} for $\epsilon_{0}$ sufficiently small. In particular, one can prove there exists a universal $M>1$, such that $E^k\le M^{-k}$ for all $k \in \N$. Passing $k \to \infty$ yields \eqref{eq:ZeroTrunc}, for $\epsilon_0$ small enough.
\end{proof}


The remainder of the proof is devoted to obtaining bounds for the Holder seminorm.
We begin by using the extension problem to reduce the Holder continuity estimate to an oscillation reduction result.  We will use $B_{r}^{*}=[-r,r]^{d}\times [0,r]$.  The main theorem can be reduced to the following proposition.
\begin{Prop}\label{prop:oscillationreduction}
There exist a positive universal constant $\lambda^*$ such that for all $\theta \in \mathcal{S}(D,\alpha)$, the following statement is true. If $\theta^{*} \leq 2$ in $B_{1}^{*}\times[1,2]$ and
\begin{equation*}
|\{(x,z,t) \in Q_{1}^{*} \mid \theta^{*}(x,z,t) \leq 0 \}| \geq \frac{1}{2}|Q_{1}^*|
\end{equation*}
then $\theta^{*} \leq 2-\lambda^*$ in $B_{r}^{*} \times [\frac{3}{2},2]$, where $r=2^{-\frac{1}{2\alpha}}$. 
\end{Prop}
From the previous proposition we have the following useful Corollary. 

\marginnote{The end point in time of the oscillation can be taken to be 2?}
\begin{Cor}\label{cor:reductionofoscillation}
There exist a positive universal constant $\mu^*<1$ such that for all $\theta \in \mathcal{S}(D,\alpha)$, the following statement is true.
\begin{equation}\label{eq:decreaseofoscillations}
\underset{[\frac{3}{2},2] \times B_{r}^{*}}{\text{osc}}\theta^{*}\le \mu^*\underset{[1,2] \times B_{1}^{*}}{\text{osc}} \theta^{*},
\end{equation}
where $r=2^{-\frac{1}{2\alpha}}$.
\end{Cor}

{\color{red} Prove Corollary!!!}
The H\"{o}lder continuity of solutions, follows by using  classical arguments.
\begin{proof}[Proof of Main Theorem~\ref{Thm:HolderContResult}]
Given $r>0$, we fix $(t_0,x_0)\in (r,\infty)\times\R^d$. We consider $k\in \N$ sufficiently large ($k>-ln_2(r/2)$), and we take the re-scaling
$$
\tilde{\theta}(\tilde{t},\tilde{x})=\theta\left(2^{-k+1}(t-7/4)+t_0,r^{k-1}x+x_0\right),
$$
which preserves $\tilde{\theta}\in \mathcal{S}(D,\alpha)$. Therefore, by Corollary~\ref{cor:reductionofoscillation}
$$
\underset{[\frac{3}{2},2] \times B_{r}^{*}}{\text{osc}}\tilde{\theta}^{*}\le \mu^*\underset{[1,2] \times B_{1}^{*}}{\text{osc}} \tilde{\theta}^{*}.
$$
Un-doing the scaling we get
$$
\underset{[t_0-2^{-k-1},t_0+2^{-k-1}] \times B_{r^k}^{*}}{\text{osc}}\theta^{*}\le \mu^*\underset{[t_0- 2^{-k-1}3,t_0+2^{-k-1}] \times B_{r^{k-1}}^{*}}{\text{osc}} \theta^{*}.
$$
Doing the previous step inductively, we get for $k_0>-ln_2(r/2)$,
\begin{equation}\label{eq:Qk0toQk}
\underset{Q_{k}}{\text{osc}}\theta\le\underset{Q_{k}^{*}}{\text{osc}}\theta^{*}\le (\mu^*)^{k-k_0}\underset{Q_{{k_0}}^{*}}{\text{osc}} \theta^{*},
\end{equation}
where $Q_k=(x_0,t_0)+B_r^k\times[-2^{-2k},2^{-2k}]$ and $Q_k^*=Q_k\times[0,r^k]$.

Finally, using the $L^2\to L^\infty$ Lemma, we know that
$$
\begin{aligned}
\underset{Q_{{k_0}}^{*}}{\text{osc}} \theta^{*}
\le 2||\theta^*||_{L^{\infty}(Q_{{k_0}}^{*})}
&\le 2||\theta^*||_{L^{\infty}(t_0-2^{-2k_0},\infty)\times\R^d\times \R_+}\\
&=2||\theta||_{L^{\infty}(t_0-2^{-2k_0},\infty)\times\R^d}
\le 2C \left(\frac{r}{2}\right)^{-2\alpha d}||\theta(0)||_{L^2(\R^d)},
\end{aligned}
$$
where we have used $k_0\ge-\ln(r/2)$ and $t_0>r$.
Combining the last inequality with \eqref{eq:Qk0toQk}, we obtain
$$
\underset{Q_{k}}{\text{osc}}\theta\le C \left(\frac{r}{2}\right)^{-2\alpha d}||\theta(0)||_{L^2(\R^d)},
$$
which proves the Theorem.



% \noindent The second step is to iterate the reduction of oscillation on all scales. By re-scaling




% We can do this by induction, we assume that 
% \begin{equation}
% \underset{Q_{k}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*} \leq (1-\lambda^{*})^{k-k_{0}}\underset{Q_{k_{0}}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*}.
% \end{equation}




% Towards this end, we fix a $t_{0}>r$ and $x_{0} \in \R^{d}$ then define a sequence of space/time cylinders by the relation $Q_{k}(t_{0},x_{0})=[t_{0}-2^{-k},t_{0}+2^{-k+1}] \times B_{r^{k-1}}(x_{0})$.  Also, let $Q_{k}^{*}(t_{0},x_{0})=Q_{k}(t_{0},x_{0}) \times [0,r^{k-1}]$.  Next we choose a sufficiently large $k_{0}$ to start the iteration from, namely $k_{0}(r)= \lceil \ln_{2}(\frac{r}{2})\rceil$.  We will verify that for all $k \geq k_{0}$,
% \begin{equation}
% \underset{Q_{k}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*} \leq (1-\lambda^{*})^{k-k_{0}}\underset{Q_{k_{0}}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*}.
% \end{equation}
% Indeed, for each $k \geq k_{0}$, define a transformation $T_{k}:\R^{d+1} \to \R^{d+1}$ via \begin{equation*}
% T_{k}(t,x)=\big[2^{-k+1}(t-1)+t_{0},r^{k-1}x + x_{0}\big].
% \end{equation*}
% Observe that $\theta \circ T_{k} \in \mathcal{S}(D,\alpha)$ and $(\theta \circ T_{k})^{*}=\theta^{*} \circ T_{k}^{*}$, where $T_{k}^{*}: \R^{d+2} \to \R^{d+2}$ is defined by 
% \begin{equation*}
% T_{k}^{*}(t,x,z)=\big[T_{k}(t,x),r^{k-1}z\big].
% \end{equation*} 
% By design, we have $T_{k}^{*} \big ( [\frac{1}{2},2] \times B_{1}^{*}\big )=Q_{k}^{*}$ and $T_{k}^{*} \big ( [\frac{3}{4},{\frac{3}{2}}] \times B_{r}^{*}\big )=Q_{k+1}^{*}$.  Thus, applying the unit scale oscillation reduction result to $\theta \circ T_{k}$ yields
% \begin{equation}
% \underset{Q_{k+1}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*} \leq (1-\lambda^{*})\underset{Q_{k}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*}.
% \end{equation}
% Iterating this inequality gives the claim.  Next observe that $k_{0}$ was chosen to ensure that for each $t_{0}\geq r$, we have $t_{0}-2^{-k} \geq \frac{r}{2}$.  Thus, we have
% \begin{equation}
% \sup_{Q_{k_{0}}^{*}(t_{0},x_{0})}|\theta^{*}| \leq \sup_{[\frac{r}{2},\infty) \times \R^{d} \times \R_{+}}|\theta^{*}| \leq \sup_{[\frac{r}{2},\infty) \times \R^{d}}|\theta| \leqs (\frac{2}{r})^{-2\alpha d},
% \end{equation}
% uniformly over $x_{0} \in \R^{d}$ and $t_{0} \geq r$.  Here, we used the $L^{2} \to L^{\infty}$ lemma together with Young's inequality and the explicit form of $\theta^{*}$.  Finally, we can obtain the decay of oscillations for $\theta$ by using $\theta^{*}(t,x,0)=\theta(t,x)$to obtain for $k \geq k_{0}$,
% \begin{align*}
% &\underset{Q_{k}(t_{0},x_{0})}{\text{osc}}\theta \leq \underset{Q_{k}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*} \leq (1-\lambda^{*})^{k-k_{0}}\underset{Q_{k_{0}}^{*}(t_{0},x_{0})}{\text{osc}}\theta^{*}\\
% &\leqs (1-\lambda^{*})^{k-k_{0}}(\frac{2}{r})^{-2\alpha d}.
% \end{align*}
\end{proof}

==> Section5_0.tex <==
%!TEX root = main.tex
In this remark, we comment on the main elements of the Di Georgi iteration step.\\  

\emph{Comparison with the Classical $L^{2} \to L^{\infty}$ Step} \\

The first point is to compare the statement itself to the more classical statement arising in elliptic and parabolic equations.  Recall that in the classical Di Georgi theory, there exists a universal $\epsilon>0$ such that if $\theta$ solves
$$
\Div(A\nabla \theta)=0
$$ 
in $B_{1}$ and $|\theta|_{L^{2}} < \epsilon$, then $\theta \leq 1$ in $B_{r}$.  ence, ideally we would like to prove the same statement, but under the hypothesis $|\theta^{*}|_{L^{2}_{t,x,z}}<\epsilon$.  Unfortunately, we cannot prove this.  

In fact, the proof relies on a delicate interplay between the usual Di Georgi nonlinear inequality and a barrier function argument.  Since we setup a barrier for certain truncations of $\theta^{*}$, we need to hypothesize a starting $L^{\infty}_{t,x,z}$ bound in order to know which barriers to select.  Thus, we need more information than smallness to get started, and we must change slightly the statement of the claim.  Namely, it is proved that under a local $L^{2}$ type smallness on $\theta^{*}$ and $\theta$, the $L^{\infty}$ bound for the solution improves as we venture inward to a smaller ball. \\

\emph{The Role of the Barrier Functions}\\

In view of the above remark, we now fix our attention on $\theta \in S(D,\alpha)$ such that $\theta^{*} \leq 2$ locally.  Three different barriers are constructed.  The purpose of the the first barrier is to prove that locally, an inequality of the following type holds:
\begin{equation} \label{Eq:B1Est}
\theta_{M}^{*} \leq (\eta \theta_{M})^{*}+b_{1}.
\end{equation}
Observe that $\theta_{M}^{*}$ and $(\eta \theta_{M})^{*}$ agree for $z=0$, so $b_{1}$ should vanish there.  On the other parts of the boundary, we use the only information we have, that $\theta_{M}^{*}\leq \theta^{*} \leq 2$, and set the barrier equal to $2$.

The purpose of the second barrier is to remove $b_{1}$ from the inequality above.  The trick is to compensate by cutting off $\theta^{*}$ at twice the height that we cutoff $\theta$ by.  That is, we seek a local ineqality of the form:
\begin{equation}
\theta_{2M}^{*} \leq (\eta \theta_{M})^{*}.
\end{equation}
Observe that the inequality is trivial if $\theta_{2M}^{*}=0$.  Otherwise, we have the identity $\theta_{2M}^{*}=\theta_{M}^{*}-M$.  Hence, subtracting $M$ from both sides of $\ref{Eq:B1Est}$, we find that
\begin{equation}
\theta_{2M}^{*} \leq (\eta \theta_{M})^{*}+(b_{2}-M).
\end{equation}
Thus, the inequality will hold as long as the truncation wipes out the barrier.

The purpose of the third barrier is to reduce the problem of showing that $\theta^{*} \leq 2-\lambda$ to showing that $\theta \leq 2-\lambda'$ for some $\lambda'>0$.  Then we put up a barrier taking the value $2$ everywhere along the box except for the bottom, where we put $2-\lambda'$, and this is sufficent to reduce $\theta^{*}$ to height $2-\lambda$. \\

\emph{Construction of the Second Barrier} \\

The idea for the construction of the second barrier is as follows.  We start by building a barrier on the unit scale.  Namely, we consider $(x,z)$ space given as $\R_{+} \times [0,1]$. Consider a barrier designed to be harmonic or pseudo harmonic on the inside with the following boundary conditions.  On the bottom, we put $0$ and on the top we put $\epsilon$.  On the left side we put the value $2$.  For this barrier, call it $b$, we have a bound(uniform in $z \in [0,1]$)
$$
b(x,z) \leq \epsilon + Ce^{-x}.
$$
Observe that this bound is only useful provided we stay sufficiently close to $x=0$.  From here, the idea is to make a transformation and build a barrier in $B_{k}^{*}=[-r-2^{-k},r+2^{-k}] \times [0,\delta^{k}]$.  Clearly, we have to dilate in $z$.  However, we want the role of the point $0$ in the unit scale to play the role of each of the lateral sides in $B_{k}^{*}$.  The top and the bottom are the same as before.  Hence, we break $B_{k}^{*}$ into a left and a right side.  For the left side, the only thing we have to do is shift everything, then rescale.  Observe that we must rescale in $x$ in the same way as we rescale in $z$ in order for the equation to still hold.  For the right side of the box, the problem is that the origin is in the wrong place.  Hence, we reflect everything first, and then shift and rescale. \\

\emph{Attempting to use an Updating Barrier Function}

One idea, was to choose $\epsilon$ according the bound we have for $\theta_{k}^{*}$ and hope that we can use the exponential decay of energy to kill the next step.  Now, we must stay sufficiently far away from the sides in order to use the exponential decay.  The idea is to restrict our attention to a smaller cube in between $B_{k}^{*}$ and $B_{k+1}^{*}$ defined by $\overline{B_{k}^{*}}=[-r-2^{-\frac{k}{2}},r+2^{-\frac{k}{2}}] \times [0,\delta^{k}]$.  In this region, denoting by $\overline{b}_{\epsilon}$ the barrier in the full cube, we get
$$
\overline{b} \leq \epsilon + Ce^{-(2\delta)^{-k}}.
$$
The idea now would be to let $\epsilon_{k}=|\eta_{k}\theta_{k}^{*}|_{L^{\infty}(B_{k} \times [\delta^{k+1},\delta^{k}])}$.  We would then obtain the following inequality:
$$
\eta_{k}\theta_{k}^{*} \leq \eta_{k} \big [ (\eta_{k}\theta_{k})^{*}+b_{\epsilon_{k}} \big]
$$
The problem is that the LHS of the inequality is not easily controlled in terms of the energy alone.  This was the same problem we had before.  \\

\emph{The Significance of the Inductive Step} \\

From the last paragraph, we saw that the key obstruction to any barrier argument is the lack of information about $\theta_{k}^{*}$ near the top of the box.  The key idea hidden in the inductive step is that it is easy to go from $2$ to $2-\tilde{\lambda}$ if we restrict our attention to $z \sim 1$.  Indeed, put up the naive barrier by localizing before extending and then adding on a barrier with 0 and then bottom and $2$ on the sides and the top.  If we move inward in $x$, then be can ensure $b \sim 2-\lambda'$.  Moreover, if $z \sim 1$, then Young's inequality tells us that extension of the localization is of order $\epsilon_{0}$.  Hence, choosing $\epsilon_{0}$ small enough relative to $\lambda'$ yields a $\tilde{\lambda}$.  Truncating by this amount wipes out $\theta_{1}^{*}$ at the top of the box.  

Hence, if we can show that this propagates as we $k \to \infty$ and we cut closer and closer to the $z=0$ border, then we can continue to use the truncation to wipe out the influence of the barrier.





\emph{Inputs to the Iteration Scheme}\\

Introduce a decreasing sequence of space/time cubes $Q_{k}=[T_{k},2]\times B_{k}$ where: 
\begin{align*}
&1\leq T_{k} \leq T_{k+1}\leq \frac{3}{2} \\
&B_{2r} \subset B_{k+1} \subset B_{k} \subset B_{1}. 
\end{align*}

Also, define cubes in extended space $B_{k}^{*}=B_{k} \times [0,z_{k}]$ for a sequence $0 \leq z_{k+1} \leq z_{k}$.  Let $Q_{k}^{*}=[T_{k},2] \times B_{k}^{*}$.

For each $k \geq 1$, construct a cutoff $\eta_{k}: \R^{d} \to [0,1]$ supported in $B_{k}$ and satisfying $\eta_{k}1_{B_{k+1}}=1$.  Let $\sigma_{k}$ be an extension of $\eta_{k}$ to $\R^{d} \times \R_{+}$ which is supported in $B_{k}^{*}$ and satisfies $\sigma_{k+1}1_{B_{k+1}^{*}}=1$.

Next, for each $k \geq 1$ define a cut $M_{k}=2-\lambda_{k}$ and the corresponding truncations $\theta_{k}=(\theta-M_{k})_{+}$, $\theta_{k}^{*}=(\theta^{*}-M_{k})_{+}$.

Finally, define the sequence of energies via
$$
E_{k}=\int_{\R^{d}}\eta_{k}\theta_{k}^{2}dx + \iint_{\R^{d} \times \R_{+}}z^{1-2\alpha}|\nabla(\sigma_{k}\theta_{k}^{*})|^{2}dxdz.\\
$$

\emph{The Smallness Condition}\\

As we discussed above, our goal is to wipe out the barrier.  However, the difference between consecutive cuts is geometric.  That is, $M_{k+1}-M_{k} \sim 2^{-k}$, which means that the barrier must be quite small.  The trick for this is to prove a support property on $\eta_{k}\theta_{k}^{*}$.  Namely, that if we make appropriate cuts, then for $z \geq \overline{z}_{k}$, this quantity vanishes.

This will allow us to use a barrier which vanishes on both the top and the bottom of the cube and can only gain energy due to the influence on the sides.  

For this purpose, we must use the smallness condition on $\theta$ again.  Intuitively, the idea is that since there is very small energy in $\theta_{k}$, the extension $\theta_{k}^{*}$ cannot be too large if we are in an intermediary regime $z \in [a,b]$ away from the border but not too far into infinity.  Quantitatively, this is built into Young's inequality:
$$
|\theta * P(z)|_{L^{\infty}_{x}} \leq |P(z)|_{L^{2}_{x}}|\theta|_{L^{2}_{x}}.
$$

\emph{Moving inward in the Extended Variable}\\

The difficulty with using the Young's inequality above is that
$$
\lim_{z \to 0} |P(z)|_{L^{2}_{x}}=\infty.
$$
Fortunately, the inequality above is actually applied to $\theta_{M}$.  If the Di Georgi scheme is working, then $|\theta_{M}|_{L^{2}_{x}}$ is converging to zero as $M$ approaches $2-\lambda$.

Hence, if we are working in a fixed region of $z$ bounded away from zero, this term could be made small by choosing the initial energy sufficiently small and using the monotonocity of the truncations.  On the other hand, if we are forced to work with a sequence $z_{k} \to 0$, then we need more than smallness of the initial energy, we need the Di Georgi scheme to be working, and we need $|\theta_{k}|_{L^{2}_{x}} \to 0$ more quickly that $|P(z_{k})|_{L^{2}_{x}} \to \infty$.

Finally, we arrive at the main issue.  Why is it necessary to take a sequence of $\{ z_{k}\}_{k=1}^{\infty}$ converging toward zero?  The issue is the following:  we will need to construct a sequence of barriers $\{ b_{k}\}_{k=1}^{\infty}$ such that $|b_{k}|_{L^{\infty}_{x,z}} \to 0$ as $k \to \infty$.  Since we have no control over what happens on the sides, the only hope is to shrink the size of the $z$ domain and automatically the influence of the barriers.  The question becomes the following: suppose we have a sequence of barrier functions which take the value $0$ at the bottom of the cube and the value $2$ on the top and the sides.  Intuitively, these barriers should converge pointwise(in $z$) to the zero boundary data.  The question is whether the convergence is locally(cutting away the boundary influence)uniform to zero or not. 


\emph{Setting the Constants}\\

Roughly, the setting of the constants is to ensure three different gates open: the first gate is the geometric decay of the energy.  The second constraint is to ensure that cutting kills the barrier.  The third constraint is to ensure that the vanishing of $\theta_{k}^{*}$ on the $z$ boundary propagates.
